Normalisation for a Neutral Free Logic with Definite Descriptions

In this paper, we present a natural deduction system for a strong Kleene-based neutral free logic with definite descriptions. The system combines a three-valued propositional basis with free quantification, identity, existence, and rules for definite descriptions. The main result is a normalisation theorem for a proof-theoretically equivalent restricted formulation of the system; we also establish a corresponding modified subformula property for its fragment.

==> eptcsdata.tex <==
\providecommand{\firstpage}{133}
\providecommand{\publicationstatus}{A. Indrzejczak, T. Jarmu\.zek, M. Klonowski, \& M. Zawidzki (Eds.):\\ Twelfth International Conference on\\ Non-Classical Logics. Theory and Applications (NCL'26)\\
EPTCS 455, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.455.11}{10.4204/EPTCS.455.11}}

